Decentralizing Platform Power: A Design Space of Multi-level Governance in Online Social Platforms

Many have criticized the centralized and unaccountable governance of prominent online social platforms, leading to renewed interest in platform governance that incorporates multiple centers of power. Decentralization of power can arise horizontally, through parallel communities, each with local administration, and vertically, through multiple hierarchies of overlapping jurisdiction. Drawing from literature on federalism and polycentricity in analogous offline institutions, we scrutinize the landscape of existing platforms through the lens of multi-level governance. Our analysis describes how online platforms incorporate varying forms and degrees of decentralized governance. In particular, we propose a framework that characterizes the general design space and the various ways that middle levels of governance vary in how they can interact with a centralized governance system above and end users below. This focus provides a starting point for new lines of inquiry between platform- and community-governance scholarship. By engaging themes of decentralization, hierarchy, power, and responsibility, while discussing concrete examples, we connect designers and theorists of online spaces.

==> 05-differences.tex <==
% \section{Discussion}

% By drawing analogies between platform governance and offline multi-level systems, we use literature on offline institutions towards a design space of multi-level governance in online social platforms. 
% We discuss some of the limits of those analogies before turning to propose design implications and further research drawing from our design dimensions to support platforms and communities seeking to decentralize their governance. 

\section{Differences in Online and Offline Multi-level Governance Systems}
\label{diff}
In the last section, we drew analogies between platform governance and offline multi-level systems towards proposing a design space of multi-level governance in online social platforms.  
While there is much we can learn from offline institutions, governing online spaces poses some unique challenges: there are fundamental ways in which social platforms differ from offline systems. 
There are also crucial ways in which offline theories of governance break analogy with governance on online platforms, and insights from the former do not translate well to the latter. 
%We elaborate on these differences and challenges below.

\subsection{Limitations of Offline Theories of Governance in Explaining Online Phenomena}
%We detail some key differences below.
%\noindent \textit{Organizational Theory}:
%While organizational theory provides valuable insights about the effects of organizational structure on decision making, it
As mentioned earlier, organizational theory tends to assume that all agents in the hierarchy are working towards the same end \citep{joseph2020organizational}. This crucial assumption helps researchers focus on how firms process information, but downplays the potential for conflict and competition.
%, which breaks analogy with most online communities. 
However much unity Wikipedians share around the encyclopedia's goals, they are also volunteers with individual motivations and, unlike employees in a company, are not paid to subordinate their personal goals to those of superiors. 
%Although Wikipedia is, at some level, an organization unified around a common goal of providing ``a free widely accessible encyclopedia,'' it is equally valid to see it 
In this view, Wikipedia can be seen as a highly contested, strategic space, whose articles are as often the result of compromise between editors in conflict as successful collaboration \citep{yasseri2012dynamics,borra2015societal}. 
Thus, administrative hierarchy is an incomplete analogy to online communities, where the motives behind multiple levels are as much about identifying, coordinating, and asserting the autonomy of many independent agents as they are about administrative decentralization and efficiency in information processing~\citep{forte2009decentralization,matias2016civic}.

%\noindent \textit{Federalism and Polycentricity:}
Moving to the political science literature on federalism and polycentricity, we find more points of overlap.
However, despite its superficial ability to capture the neatly nested jurisdictions observed online, federalism provides an incomplete source of properties general enough to illuminate multi-level governance online. First, its focus on nation-scale federations comes almost entirely at the expense of other scales of governance systems.  This results in a narrow view, evidenced by some of the criteria political scientists have used to taxonomize federations, such as a formal distribution of legislative and executive authority, a supreme written constitution, and a system of courts~\citep{loughlin2013routledge}. These criteria are much too onerous to describe the kinds of multi-level platforms that we observe. \citet{aroney2016types} offers a taxonomy of multi-level governance systems that is more general, but still nation-focused. Polycentricity offers a framework better suited to platform governance but assumes the presence of ``critical supporting roles'' \citep{mcginnis2012reflections,ostrom1961organization} that have no analogues in online platforms.

\subsection{Stakes Involved in Online Governance are Qualitatively Different}
While online governance focuses on activities such as information sharing and building social capital, offline governance deals with a wider set of issues, including protecting from external physical threats and ensuring the overall welfare of citizens.
% The stakes involved in platform governance are very different than those for offline governance. 
Further, individuals have higher mobility online than in offline settings, and the constraints for entry/exit are lower. This shapes the perspectives and practices of stakeholders on digital platforms. We note that important exceptions exist: for instance, users who rely on online support groups for mental health help, LGBT issues, \textit{etc}., may highly depend on the social support offered by online communities \citep{kiesler2012}. Still, democratic participation in governance is rare online. The private ownership of most online platforms means that the financial benefits of good governance are not necessarily reinvested in improving community outcomes, further discouraging public participation in governance online. 




\subsection{Compensation of Labor}
While offline administrators in governance centers at different levels are supported through tax dollars, online administrators in middle-level units are typically volunteer contributors with lower support from top and bottom levels, as shown in Table~\ref{table:cross-level}.
Researchers have highlighted the significant labor that goes into enacting content moderation~\citep{wohn2019volunteer,jhaver2019automated,roberts2019behind,gray2019ghost}. 
% Even in the cases of industrial content moderation that is paid for by platforms, moderators receive low wages and no mental health support in return for reviewing psychologically damaging content~\citep{roberts2019behind,gray2019ghost}.
This discrepancy raises the question of whether local content moderators should receive financial compensation for the responsibilities they shoulder. 
Few platforms have explored alternative business models for compensating local administrators, which could involve anything from the sharing of ad revenue with lower-level administrators, to subscription-based models that support local and global governance, to even multi-stakeholder ownership of platforms~\citep{schneider2020exit}.
%Hiring an increasing number of moderators to curate content may become prohibitively expensive at some stage \citep{masnick_2019}.
%As the legal and public pressure on large platforms increase, they would increasingly need to acknowledge the failures of their current centralized moderation processes. 
 %Thus, it may benefit platforms to rely on lower-level governance units and share in their ad revenue with administrators at those levels. 
 Some scholars have proposed a marketplace of governance services separate from platforms, analogous to emergent middle levels in our design space~\citep{masnick_2019,wolfram_2019,2021-modpol,esber2021meta}, though it remains an open question how third-party services themselves will have viable business models~\citep{marechal2021future}. 
%Having such a marketplace would open up alternative ways of compensating for moderation labor.
%However, some critics have argued that having such a marketplace would put the onus on end-users to protect themselves from online abuse by subscribing to such services and abdicate platforms from protecting consumers \citep{gault2021Intel}.

\subsection{Decisions about Technical Architecture Shape Middle Levels}
Unlike offline institutions, each platform makes a whole host of technical decisions that affects whether middle levels emerge and how they behave. 
%Such decisions include whether to host platform data on a private server or a cloud service or whether the platform enforces standards for interoperability. If the latter case is true, the middle levels of governance are bound to exist. On the other hand, centralized platforms with no interoperability standards do not necessarily have to support middle levels.
One key infrastructural decision that affects the emergence of middle levels is whether a platform provides external access through an API. 
With sufficient access, third-party middle levels like Twitter blocklists can emerge. However, these middle levels have a precarious existence and can be deliberately shut down or inadvertently broken by changes in the API. 
Similarly, if a platform abides by an interoperable standard, then middle levels are bound to exist, though they may be highly unequal in membership.
Mastodon demonstrates how architecture can shape middle levels: nodes are self-hosted, with a thin top level consisting of a common technical standard. While nodes are somewhat constrained by the code implementing the standard, they can also fork this code and govern themselves in different ways.
We note that while technical constraints can powerfully influence governance, scholars have repeatedly demonstrated how an over-reliance on technical decentralization can merely exchange the formal endowment of central powers with an emergent rise of central powers~\citep{de2016invisible,raman2019challenges,barbereau2022defi}.
While some degree of inequality is to be expected, future work is needed to more carefully recognize  emergent centralization in multi-level governance platforms, using metrics such as the Gini coefficient on membership size of different middle level units along with our design dimensions. 

Another example of how technical decisions can constrain or empower decentralized governance is of WhatsApp enforcing end-to-end encryption for its chats. This precludes the top level from directly taking governance actions on end users or from overseeing middle levels. It also empowers WhatsApp Group admins, who form the middle level of WhatsApp governance, to have greater autonomy.



% In some cases, platforms choose to institute asymmetric governance levels that privilege certain governance units over others. Such disparate treatments can create resentments and lead to inter-level conflicts. For example, when YouTube enforced its content take-down and demonetization policies differently for different types of channels, it resulted in a backlash from amateur creators against the site \citep{caplan2020tiered}.





% \subsection{Policy Recommendations}
% While hierarchical governance structures provide an array of benefits over the centralized systems as detailed above, they also are vulnerable to being abused. Take the example of Twitter blocklists. While these blocklists were developed to prevent online harassment, we found that the terrorist group Islamic State of Iraq and the Levant (ISIL/ISIS) uses blocklists as part of its web communication strategy \citep{jhaver2018blocklists}. It maintains a number of blocklists at any given time that block users who tweet anti-ISIS posts or engage in combating ISIS on Twitter. We suspect that ISIS may be asking users in early stages of radicalization to subscribe to these blocklists, so that they may access only the pro-ISIS rhetoric. Therefore, ISIS could be using these blocklists to appropriate Twitter as a safe space and promote its ideology.
% Previous research has shown that “users often appropriate and adapt technology in ways never envisaged by the designers” \citep{dix2007}. The creators of blocklists probably could not have envisioned that this technology would be used to assist ISIS radicalization.

% Another key issue is the embedding of biases within lower-level governance units. For example, some subreddits may want to systematically exclude certain voices and configure Automod to enable such exclusion, but no oversight currently exists to discourage this. Specific instances of word filters or blocklists may have poor accuracy and censor appropriate posts inadvertently, but it may be hard to know that this is even happening and correct for it. Since these tools are privately configured and used, they cannot be transparently or publicly audited. 

% One solution could be create an intermediate layer of governance units that regularly evaluate the operations of lower-level governance units under its jurisdiction. For example, a governance unit could be created to manage the blocklist app, and it could be responsible for ensuring that all instances of Twitter blocklists operate appropriately. 
% Such an oversight would help ensure that lower-level governance units do not create systematic biases or promote toxic content. At the same time, platforms should be proactive in ensuring that governance units operate well. Platforms should offer not just a one-time approval and access to these units, but also expect unit administrators to submit regular summarized reports on how they are operating, the problems they have identified, and the steps they have taken to resolve them. Platforms could also build live analytic tools that provide them visibility into the key metrics of their lower layers' operations. This double layer of regulated markets would ensure that platforms are not overwhelmed with regulating each instance of a wide variety of tools, but they have the power to stop the use of a tool if it does more harm than good. Platforms should also create a separate reporting mechanism for end-users to directly report their dissatisfaction with any governance unit. Further, researchers, activists, and journalists should also have visibility into the operation of these units.


% \subsection{Time/Community Lifecycle?}

% emergent centralization in decentralized systems and entrenchment of powers

% Mako's iron law of oligarchy

% beginning of the community lifecycle vs growth stage (production) vs stable period (moderation)

% \subsection{Future Directions for Research}


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

